Automatic inference of fault tree models via multi-objective evolutionary algorithms

Fault tree analysis is a well-known technique in reliability engineering and risk assessment, which supports decision-making processes and the management of complex systems. Traditionally, fault tree (FT) models are built manually together with domain experts, considered a time-consuming process prone to human errors. With Industry 4.0, there is an increasing availability of inspection and monitoring data, making techniques that enable knowledge extraction from large data sets relevant. Thus, our goal with this work is to propose a data-driven approach to infer efficient FT structures that achieve a complete representation of the failure mechanisms contained in the failure data set without human intervention. Our algorithm, the FT-MOEA, based on multi-objective evolutionary algorithms, enables the simultaneous optimization of different relevant metrics such as the FT size, the error computed based on the failure data set and the Minimal Cut Sets. Our results show that, for six case studies from the literature, our approach successfully achieved automatic, efficient, and consistent inference of the associated FT models. We also present the results of a parametric analysis that tests our algorithm for different relevant conditions that influence its performance, as well as an overview of the data-driven methods used to automatically infer FT models.

==> Figures/FWKjaRgchx_parametric_case_studies.tex <==
\begin{figure}[!h]
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_case_studies/pop_400_acc_data.pdf}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_case_studies/pop_400_acc_mcs.pdf}
  \caption{}
\end{subfigure}%

\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_case_studies/pop_400_tree_size.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_case_studies/pop_400_time.pdf}
  \caption{}
\end{subfigure}
\caption{Comparing the performance of the o.f's $\Phi(+\phi_c,-\phi_s,+\phi_d)$ and $\Phi(0,0,+\phi_d)$ for all the case studies in Table \ref{tb:case_studies}, using $ps=400$, $ng=100$, $uc=20$. In (a) accuracy of the outputting fault tree based on the fault data set ($\phi_d$), (b) accuracy of the outputting fault tree based on the MCSs ($\phi_c$), (c) size of the outputting fault tree ($\phi_s$), and (d) convergence time.}
\label{fig:FWKjaRgchx_parametric_case_studies}
\end{figure}

==> Figures/aShO3Uk0W6_noise_per_case_study_per_obj_function.tex <==
\begin{figure*}[!h]
\centering
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_MPPS_sd.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_MPPS_sc.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_MPPS_cd.pdf}
  \caption{}
\end{subfigure}

\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_ddFT_sd.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_ddFT_sc.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_ddFT_cd.pdf}
  \caption{}
\end{subfigure}

\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_Covid-19_sd.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_Covid-19_sc.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.31\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/comparing_noise_obj_functions_case_study/pop_400_Covid-19_cd.pdf}
  \caption{}
\end{subfigure}

\caption{Metrics under the influence of noise for two m.o.f.'s namely \textit{sd} (triangles) and \textit{d} (circles), the size of the markers is proportional to the number of repetitions. Using $ps=400$, $ng=100$, $uc=20$. Case studies: (a)(b)(c) MPPS, (d)(e)(f)  ddFT, and (g)(h)(i) Covid-19. In (a)(d)(g) error based on the fault data set ($\phi_d$) versus fault tree size ($\phi_s$), (b)(e)(h) error based on the MCSs ($\phi_c$) versus fault tree size ($\phi_s$), (c)(f)(i) error based on the fault data set ($\phi_d$) versus the error based on the MCSs ($\phi_c$). The color bar is associated to the noise levels $n_0=0\%$, $n_10=10\%$, $n_20=20\%$.}
\label{fig:aShO3Uk0W6_noise_per_case_study_per_obj_function}
\end{figure*}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}

%\begin{itemize}
%    \item Our approach performed faster when minimizing the size of the trees between generations.
%    \item When accounting for the MCSs as part of the multi-objective function, positively impacted the data-driven inference of fault trees from data.
%    \item Our approach works as a compressor of fault trees.
%    \item We propose three categories to classify the type of approaches, and add an overview on data-driven methods (this is a contribution).
%\end{itemize}


% We observe how consistent the FT-MOEA is when converging to the same result for most of the cases.

% Our algorithm works as a compressor of FT models.


In this paper, we addressed the issue of automatically inferring fault trees (FTs) from noise-free and complete failure data sets via a multi-objective evolutionary algorithm based on the Elitist Non-Dominated Sorting Genetic algorithm (NSGA-II) and Crowding-Distance. We successfully showed that it is possible to achieve consistently efficient FT structures in a data-driven manner.

As part of our parametric analysis, we used as ground truth diverse FTs from the literature. We observe that our algorithm, the FT-MOEA, has in general a better performance than the predecessor, the FT-GA. Our algorithm accounts for three parameters in the multi-objective function (m.o.f.) namely the size of the FT, the error based on the failure data set, and the error based on Minimal Cut Sets (MCSs).

From the parametric analysis, we can conclude that the use of larger population sizes increases the chances of finding the global optimum but makes the algorithm slower. We observe that the m.o.f. $sdc$ outperformed in most cases the other configurations by converging faster, inferring compact FT structures, achieving lower errors, being consistent and insusceptible to the presence of superfluous variables.

%Regarding the variation of the parent FTs we observe that they set different starting points, the approach using two parent FTs, one with a single $And$ gate, and the other with a single $O$ gate is faster compared to using the disjunctive normal form, but we believe that this can be improved by enhancing the way the MCSs are currently computed. We note that our algorithm is able to handle and eliminate spurious variables in the failure data set.

% We also provided a qualitative comparison with state-of-the art algorithms that infer FTs in a data-driven manner, showing several benefits and drawbacks. We believe that making a quantitative comparison is relevant to get more insights on their performances. We have identified as main limitation and future research the ones associated to scalability, which arguably can be improved by means of ``guided'' multi-objective evolutionary algorithms, Bayesian probability logic, and machine and deep learning-based approaches.

%TODO: Add that FT-MOEA is flexible, and that a similar methodology can be used to learn other type of reliability models.





==> Sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}

% What have you achieved?
We met our goal of coming up with an approach to infer efficient and interpretable FT structures that achieve a complete representation of the failure mechanisms, as well as correspond to a failure data set. We successfully achieved this by implementing multi-objective evolutionary algorithms. 

In Section \ref{sec:comp_metrics} we presented the metrics we consider within our m.o.f. (i.e., $\FTSize$, $\ErrorData$, and $\ErrorMCSs$). We observed that when minimizing $\FTSize$, the inferred FTs had indeed fewer elements compared to the cases where $\FTSize$ was not considered in the m.o.f. Our results show that our approach works as a compressor technique of FT models, with the downside of losing information associated with the intermediate events.

We observed that the inclusion of the MCSs within the optimization process greatly improved the chances of finding the global optima. However, we observed that computing the MCSs is expensive (especially for large FTs) and therefore it is necessary to look for alternatives that help to reduce this computational time. Additionally, we found that $\ErrorMCSs$ is a better measure of error than the $\ErrorData$, since the latter greatly depends on the available information in the failure data set, and the former is computed over the MCSs, which is information that better described the failure propagation in the systems.

From our parametric analysis presented in Section \ref{sec:parametric_analysis} we can make the following remarks (i) the use of large population sizes increases the chances of finding global optima and converging to the same FT model. However, this increases exponentially the computational time; (ii) for most of the case studies, the use of the m.o.f. \textit{sdc} outperformed the other m.o.f's by converging faster, inferring compact FT structures, achieving lower errors, removing superfluous variables, and being consistent.

%\begin{itemize}

%\item \item 
%\item From the different m.o.f.’s we can clearly observe the effects of minimizing the size of the FT ($\phi_s$), for all the cases, the outputting FT had smaller sizes compared to the others. The m.o.f. \textit{sdc} for most of the cases converged faster, with smaller $\phi_s$, $\phi_c$ and $\phi_d$.
%\item Regarding the relationship between the \textit{complexity} of the underlying FT for a given problem and the time that takes the algorithm to converge, we believe that this is mainly ruled by the number of MCSs involved in the problem and their orders. We also believe that research is necessary to further expand this concept.

% \item When considering \textit{superfluous variables} in the MPPS case study, we observed that the m.o.f. $sdc$ was not affected, converging 91\% of the times in the global optima, in contrast, the m.o.f. $d$ converged 23\% of the times in the global optima. The latter provides insights that our algorithm is robust and consistent. It might be worth to explore this aspect with other case studies.
% Using the m.o.f. $sdc$ it just achieved 23% of the times the global optima.

%\item When \textit{varying the parent FTs} we aimed at understanding the effects of using different starting points on the convergence process. We observed that when using the m.o.f. $sdc$, the FT-MOEA was consistently arriving to the same FT model despite the parent FT. We also observed that initializing the process with a large FT affects negatively the convergence time, since computing MCSs in large FTs is computationally expensive. We believe it is worthy to explore alternatives that allows faster computations of MCSs of large FTs and finding ways to set parent FTs that speed up the convergence process.

%\end{itemize}






==> Sections/future_research.tex <==
\section{Future Research}\label{sec:future_research}

% These are the main questions to be answered in this section:

% To what extend did you meet the goal of this paper?

% What limitations have you identified?

% From the above, what kind of aspects are relevant to further push those limitations? And what is the associated research field/line (if any).

The main drawback of our algorithm is the \textit{scalability}, this is because real-world complex systems encompass a large number of variables, exponentially increasing the size of the solution space. This makes our algorithm gets \textit{lost} among the amount of trial and error needed to achieve the global optima. We believe that a way to overcome this drawback is by means of "\textit{guided}" \textit{multi-objective evolutionary algorithms}. This concept consists of helping the optimization process by injecting additional knowledge. One way to address this is by searching out for \textit{patterns} (e.g., Waghen \& Ouali (2021) \cite{waghen2021multi}) in the failure data set that enables identifying parts of the FT (similar to the concept of Mini FTs first proposed by Powers \& Tompkins \cite{powers1974fault} back in 1973), and then assemble them. 

Another way is by \textit{guiding} the application of the \textit{genetic operators}, since currently these are randomly applied, we believe that one can increase the chances of finding the global optima by targeting and focus on parts of the FT that most likely need to be modified. The latter might be possible to achieve by implementing Bayesian probability logic. A more challenging path is exploring deep learning-based approaches like the one by Cranmer et al. (2020) \cite{cranmer2020discovering} to uncover complex relations using Graph Neural Networks. A question here is whether it is possible to use this knowledge to build system-level models.

Regarding the MOEA, we observed that by minimizing our metrics $\FTSize$, $\ErrorData$ and $\ErrorMCSs$, tiny FTs were maintained throughout the generations, this is because these FTs met the criterion of being minimal in $\FTSize$. However, these FTs commonly have high errors based on both $\ErrorData$ and $\ErrorMCSs$, making the optimization process sub-optimal. Therefore, exploring strategies that effectively address this issue are relevant.%, for example, by assessing different \textit{selection strategies} and multi-objective evolutionary algorithms. In addition, exploring this path may encounter better insights on which approach is more computational efficient.

We found that the inclusion of MCSs in the m.o.f. greatly improves the optimization process. However, as mentioned in Section \ref{sec:comp_metrics}, the FT-MOEA computes the MCSs based on the disjunctive normal form, which is computationally expensive for large FTs. Moreover, MCSs cannot be computed in noisy data. Thus, alternatives to overcome these issues are worth exploring and implement. Finally, some spare but equally interesting challenges are enlisted next.


% Regarding the efficiency of the FT structure, incorporating k/N gates within the optimization process is a good direction. As done by Lazarova-Molnaretal (2020) \cite{Feng2020DATADRIVENFT}, they use, among others, Boolean algebra, to identify logic gates in the FT. Moreover, a way to request the formation of pre-identified intermediate events within the optimization might be relevant to explore. Finally, some spare but equally interesting challenges are enlisted next.

\begin{itemize}

    \item Incompleteness in failure data sets yields into partial FT models. Thus, a question is \textit{how to handle incomplete failure data sets?} 
    
    %\item As already discussed, our m.o.f. $sdc$ can only be applied under the case of noise-free data, the reason is because the method we use to find MCSs fail when dealing with noisy data. Thus, a questions here is \textit{how to find MCSs based on noisy data ensuring the monotonicity property and completeness?}
    
    \item Many real-world problems can be considered as to be symmetric. This property could be used as an advantage, because we think this can reduce the solution space, expecting faster convergence. Thus, a question here is \textit{how to harness symmetry in the inference of FTs?}
    
    \item As pointed out by Waghen \& Ouali \cite{waghen2021multi}. Exploring alternatives of learning FTs for more complex dynamic systems, for example, where more sophisticated gates are needed (e.g., k/N gates). Research in this direction is very limited. %or when updating the FT model over time as the system ages is needed. Research in this direction is very limited.
    
    \item A more thorough comparison between different data-driven algorithms to infer FTs is needed to have a better understanding of their performances.

	\item Evaluate to what extend other multi-objective optimization algorithms improve the inference process such as the NSGA-III \cite{deb2013evolutionary}, which seems to have a better performance than the predecessor, the NSGA-II \cite{ciro2016nsga,marti2017impact}.

	%\item In Long et al. (2021) \cite{long2021non} is presented a numerical comparison between non-dominated sorting methods, they found out that \textit{dominance degree sorting} outperforms most of the methods. Thus, it may be worthy to explore solutions in this direction to see whether the optimization process can be improved.
	
	%\item It is worth exploring alternatives that enable inferring other types of logic (e.g., k/N gates), since this will yield in more efficient FT structures.
    
\end{itemize}

==> Sections/state_of_the_art.tex <==
% --------------------------------------------------- %
\section{Automatic inference of fault tree models: an overview of data-driven methods}\label{sec:state_of_the_art_algorithms}

%The automatic inference (also referred to in the literature as construction \cite{salem1976computer}, synthesis \cite{hunt1993propagation}, or induction \cite{madden1970generation}) of FT models corresponds to the task of uncovering the structure (also called skeleton\cite{linard2019fault}) of an FT from a compatible source of information. The topic of automatic inference of FT models has been discussed since the '70s, about a decade after the birth of FTs.

%Different ways of inferring FTs have been discussed in the past. We identify three main groups namely \textit{knowledge-based}, \textit{model-based}, and \textit{data-driven}. The main differences between these categories are that \textit{knowledge-based} approaches employ different heuristics for knowledge representation, using information about the basic components and their interconnections in the system under analysis \cite{latif2002comparing}; \textit{model-based} approaches translate existing system and/or graph models into FTs, and \textit{data-driven} has structured databases as a primary source of information.

%Carpignano \& Poucet (1994) \cite{carpignano1994computer}, is thoroughly reviewed several knowledge-based approaches. An example of a model-based approach can be found in Mhenni et al. (2014) \cite{mhenni2014automatic} where the authors used a SysML System Models as a base to obtain FT models. However, a major drawback of model-based approaches is the need for a pre-existing model \cite{dickerson2018formal}.


We focus our attention on \textit{data-driven} approaches. Applications of machine learning techniques and data analytics fall into this category. In Appendix \ref{app:ddFTs_table}, Table \ref{tb:state_of_the_art_literature} (divided into two parts) we summarise relevant literature in data-driven methods for the automatic inference of FT models. Below we briefly discuss these methods.

%We focus our attention on the \textit{data-driven} approaches, the main difference of this category with respect to the others is that in this case, structured data must be part of the algorithm input. Here the whole task becomes how to build an FT model that best reflects the information contained in such data set. Applications of machine learning techniques and data analytics fall into this category. In the Appendix \ref{app:ddFTs_table}, Table \ref{tb:state_of_the_art_literature} (divided in two parts) we summarise relevant literature in data-driven methods for the automatic inference of FT models. Here one can find the references, the name of the algorithm (if any), whether it is publicly available, if `yes' the table provides a hyperlink redirecting to the respective online repository. We also shortly provide some benefits and limitations per method.

%To the best of our knowledge, the very first attempt to tackle the challenge in a data-driven manner was made by Madden \& Nolan (1993) \cite{madden1970generation} with their IFT algorithm, which is based on Quinlan's ID3 algorithm to induce Decision Trees (DTs) \cite{quinlan1986induction}. The authors also continued with this work in the subsequent years \cite{madden1970hierarchically, madden1999monitoring}. In the same direction, Berikov (2004) \cite{berikov2004fault} further discusses the application of DTs to infer FTs. Mukherjee \& Chakraborty (2007) \cite{mukherjee2007automated} addressed this challenge via \textit{linguistic analysis} and domain knowledge to identify the nature of the failure from short plain text descriptions of equipment faults, and from this generate an FT model. Roth et al. \cite{roth2015integrated} propose a method that follows the Structural Complexity Management (StCM) methodology, combining the concepts of Design Structure Matrix and Domain Mapping Matrix in Multiple Domain Matrix, where their main goal is to deduce dependencies that latter on are used to infer the Boolean logic operators of the FT models. Inspired by \textit{Causal Decision Trees} \cite{li2016causal}, in Nauta (2018) \cite{nauta2018lift} they proposed an approach based on the \textit{Mantel-Haenszel} statistical test. 

To the best of our knowledge, the very first attempt to tackle the challenge in a data-driven manner was made by Madden \& Nolan (1993) \cite{madden1970generation} with their IFT algorithm, which is based on Quinlan's ID3 algorithm to induce Decision Trees (DTs) \cite{quinlan1986induction}. The authors also continued with this work in the subsequent years \cite{madden1970hierarchically, madden1999monitoring}. Mukherjee \& Chakraborty (2007) \cite{mukherjee2007automated} addressed this challenge via \textit{linguistic analysis} and domain knowledge to identify the nature of the failure from short plain text descriptions of equipment faults, and from this generate an FT model. Roth et al. \cite{roth2015integrated} propose a method that follows the Structural Complexity Management (StCM) methodology, where their main goal is to deduce dependencies that are later on are used to infer the Boolean logic operators of the FT models. Inspired by \textit{Causal Decision Trees} \cite{li2016causal}, in Nauta (2018) \cite{nauta2018lift} they proposed an approach based on the \textit{Mantel-Haenszel} statistical test.

Based on \textit{Knowledge Discovery in Data set}, Waghen \& Ouali (2019) \cite{waghen2019interpretable} propose a method for hierarchical causality analysis called \textit{Interpretable Logic Tree Analysis} (ILTA), that looks for patterns in a data set which are translated into \textit{Interpretable Logic Trees}. The first attempt based on \textit{evolutionary algorithms} was carried out by Linard et al. (2019) \cite{linard2019fault}, here the authors created an algorithm to generate FT models from a labeled binary failure data set based on a uni-dimensional cost function. Linard et al. \cite{linard2019induction} (2020) proposed a method that consisted of learning a \textit{Bayesian Network} graph, which is later translated into an FT model. Lazarova-Molnaretal (2020) \cite{Feng2020DATADRIVENFT} presents an approach based on time series of fault data, binarization techniques, MCSs, and Boolean algebra. This algorithm also manages to infer FT models with k/N logic gates. In Waghen \& Ouali (2021) \cite{waghen2021multi} the authors further extended their work to the \textit{Multi-level Interpretable Logic Tree Analysis} (MILTA), which tackles the problem of multiple cause-and-effect sequences (the latter a limitation of their previous version, the ILTA algorithm) by incorporating Bayesian probability rules.



==> Tables/case_studies.tex <==
\begin{table*}[ht]
\centering
  \begin{threeparttable}
    \caption{Case studies and associated relevant information. Number of: unique BEs ($w$), total BEs ($W$), AND gates (\#AND), OR gates (\#OR), VOT gates (\#VOT), Minimal Cut Sets (\#MCS), and order of MCSs (O-MCSs).\hl{Fix the caption.}}
     \begin{tabular}{@{}lllllllll@{}}
        \toprule
        \textit{Case study} & $w$ & $W$ & \textit{\#AND} & \textit{\#OR} & \textit{\#k/N} & \textit{\#MCSs} & \textit{O-MCSs} \\ \midrule
        CSD      & 6 & 6  & 2 & 2 & 0 & 3      & \{2,3,3\}  \\
        PT      & 6 & 6  & 1 & 4 & 0 & 5       & \{1,1,2,2,2\}  \\
        Covid-19 & 9 & 21 & 9 & 3 & 0 & 6      & \{3,4,4,4,4,4\}  \\
        ddFT      & 8 & 8 & 3 & 1 & 1 & 6      & \{3,4,4,5,6,6\}  \\
        MPPS    & 8 & 12  & 3 & 8 & 0 & 7      & \{2,2,2,2,2,2,2\}  \\
        SMS      & 13 & 17 & 0  & 8 & 0 & 13   & \{1,1,1,1,1,1,1,1,1,1,1,1,1\}  \\
        MASS     & 40 & 40 & 12 & 11 & 0 & 24  & - \\
        D2       & - & 15 & - & - & 0 & 54     & -\\ \bottomrule
     \end{tabular}\label{tb:case_studies}
    \begin{tablenotes}
      \small
      \item Container Seal Design (\textbf{CSD}) \cite{stamatelatos2002fault}; Pressure Tank (\textbf{PT}) \cite{stamatelatos2002fault}; COVID-19 infection risk (\textbf{Covid-19}) \cite{bakeli2020covid}; Data-driven Fault Tree (\textbf{ddFT}) \cite{Feng2020DATADRIVENFT}; Mono-propellant propulsion system (\textbf{MPPS}) \cite{stamatelatos2002fault}; Spread Monitoring System (\textbf{SMS}) \cite{mentes2011application}; Maritime Autonomous Surface Ships (\textbf{MASS} \cite{leefault}); Truss bridge D2 (\textbf{D2}).
    \end{tablenotes}
  \end{threeparttable}
\end{table*}

==> Tables/possibilities_objective_function.tex <==
\begin{table}[!h]
\centering
  \begin{threeparttable}
    \caption{Case studies.}
     \begin{tabular}{@{}llllll@{}}
        \toprule
        \textbf{Case} & \textbf{Acc_{data}} & \textbf{Acc_{MCS}}} & \textbf{Tree Size} \\ 
        \midrule
        CSD      & 6/6  & 2 & 2 & 0 & 3 \\
        PT      & 6/6  & 1 & 4 & 0 & 5 \\ 
        Covid-19 & 9/21 & 9 & 3 & 0 & 6\\
        DFT      & 8/8 & 3 & 1 & 1 & 6\\
        MMPPS    & 8/12  & 3 & 8 & 0 & 7 \\
        SMS      & 13/17 & 0 & 8 & 0 & 13\\
        D2       & -/15 & - & - & 0 & 54\\ \bottomrule
     \end{tabular}\label{tb:case_studies}
    \begin{tablenotes}
      \small
      \item Container Seal Design (\textbf{CSD}) \cite{stamatelatos2002fault}; Pressure Tank (\textbf{PT}) \cite{stamatelatos2002fault}; COVID-19 infection risk (\textbf{Covid-19}) \cite{bakeli2020covid}; Data-driven Fault Tree (\textbf{DFT}) \cite{Feng2020DATADRIVENFT}; Mono-propellant propulsion system (\textbf{MPPS}) \cite{stamatelatos2002fault}; Spread Monitoring System (\textbf{SMS}) \cite{mentes2011application}, Truss bridge D2 (\textbf{D2}).
    \end{tablenotes}
  \end{threeparttable}
\end{table}

==> Tables/review_early_methods.tex <==
\begin{table}[ht]\setlength\tabcolsep{2pt} 
\centering
\small

\caption{\textit{Knowledge-based} approaches for the automatic inference of FT models. In the columns the references and key aspects of the methodology.}
 \begin{tabular}{p{0.16\textwidth}p{0.30\textwidth}}
    \toprule
    \textit{Reference(s)}  & \textit{Methodology} \\ \midrule
    Fussell (1972) \cite{fussell1973formal}  & Synthetic Tree Model + Failure Transfer Functions  \\
    Powers \& Tompkins (1973) \cite{powers1974fault}  & System description + Mini FTs  \\
    Salem et al. (1976) \cite{salem1976computer}  & Decision Tables + System topological description + Backtracking \\  
    Taylor (1982) \cite{taylor1982algorithm}  & Decision Tables + Mini FTs + P\&ID  \\
    Poucet (1983) \cite{poucet1983computer}  & Macro Component Models (MCM) + Transfer Logic Models (TLM) + Human knowledge \\  
    Kelly \& Lee (1986) \cite{kelly1986propagation}    & Decision Tables + Mini FTs + Manual Feedback \\
    Wang \& Liu (1993) \cite{wang1993component}  & Decision Tables + Virtual Transfer Component + Pruning procedures  \\
    Xie et al. (1993) \cite{xie1993tree}  & Knowledge Tree + P\&ID \\  
    Hunt et al. (1993) \cite{hunt1993propagation}  & P\&ID + Mini FTs + Propagation functions \\  
    Elliott (1994) \cite{elliott1994computer}  & Graphical Function Block Diagram + Pruning techniques\\  
    Henry \& Andrews (1997) \cite{henry1997computerized}  & Digraph and Decision Tables methods \\ 
    Szabó \& Tarnai (2000) \cite{szabo2000automatic}  & Based on functional hardware and software descriptions \\ 
    Papadopoulos et al. (2001) \cite{papadopoulos2001analysis}  & Failure Functional Analysis + Failure Mode and Effect Analysis \\ 
    Majdara \& Wakabayashi (2009) \cite{majdara2009component,majdara2009new} & Component based approach: Function tables and/or State Transition Table (similar to decision tables) \\
      \bottomrule
 \end{tabular}\label{tb:review_early_approaches}
\end{table}




==> Tables/review_mbse_methods.tex <==
\begin{table}[ht]\setlength\tabcolsep{2pt} 
\centering
\small
\caption{\textit{Model-based} approaches for the automatic inference of FT models. In the columns the references and key aspects of the model source.}
 \begin{tabular}{p{0.24\textwidth}p{0.23\textwidth}}
    \toprule
    \textit{Reference(s)} & \textit{Model source} \\ \midrule
    Lapp \& Powers (1977) \cite{lapp1977computer}, de Vries (1990) \cite{de1990automated}, Andrews \& Brennan (1990)  & Digraphs  \\
    Liggesmeyer \& Rothfelder (1998) \cite{liggesmeyer1998improving} & Finite state machines \\
    Wang et al. (2002) \cite{wang2002new} & System block diagram \\
    Joshi et al. (2007) \cite{joshi2007automatic}  & AADL models \\
    Hussain \& Eschbach (2010) \cite{hussain2010automated} & Sequence-based specification (SBS) + Model testing \\
    Majdara \& Wakabayashi (2010) \cite{majdara2010computerized}  & Component-based method: + Function Table + State Transition Table + Trace-back algorithm \\
    Xiang et al. (2011) \cite{xiang2011automatic} & SysML models \\
    Mahmud \& Mian (2013) \cite{mahmud2013automatic} & AADL models \\
    Mhenni et al. (2014) \cite{mhenni2014automatic} & SysML models \\
    Herbert \& Sharp (2014) \cite{herbert2014workflow} & Model checking \\
    Mohrle et al. (2015) \cite{mohrle2015automated} & Component Fault Trees \\
    Zhang et al. (2015) \cite{zhang2015method} & Go models \\
    Iyenghar et al. (2016) \cite{iyenghar2016novel} & Simulink models \\
    Dickerson et al. (2018) \cite{dickerson2018formal} & UML activity model \\
    Wang et al. (2018) \cite{wang2018automated} & Kripke structure + Feature-Labeled Transition System (FLTS) \\
    Linard et al. (2019) \cite{linard2019induction} & Bayesian Networks \\
    \bottomrule
 \end{tabular}\label{tb:review_mbse_methods}
\end{table}









